OSM-tree: A Sortedness-Aware Index

Indexes facilitate efficient querying when the selection predicate is on an indexed key. As a result, when loading data, if we anticipate future selective (point or range) queries, we typically maintain an index that is gradually populated as new data is ingested. In that respect, indexing can be perceived as the process of adding structure to an incoming, otherwise unsorted, data collection. The process of adding structure comes at a cost, as instead of simply appending incoming data, every new entry is inserted into the index. If the data ingestion order matches the indexed attribute order, the ingestion cost is entirely redundant and can be avoided (e.g., via bulk loading in a B+-tree). However, state-of-the-art index designs do not benefit when data is ingested in an order that is close to being sorted but not fully sorted. In this paper, we study how indexes can benefit from partial data sortedness or near-sortedness, and we propose an ensemble of techniques that combine bulk loading, index appends, variable node fill/split factor, and buffering, to optimize the ingestion cost of a tree index in presence of partial data sortedness. We further augment the proposed design with necessary metadata structures to ensure competitive read performance. We apply the proposed design paradigm on a state-of-the-art B+-tree, and we propose the Ordered Sort-Merge tree (OSM-tree). OSM-tree outperforms the state of the art by up to 8.8x in ingestion performance in the presence of sortedness, while falling back to a B+-tree's ingestion performance when data is scrambled. OSM-tree offers competitive query performance, leading to performance benefits between 28% and 5x for mixed read/write workloads.

==> Makefile <==
whoami := $(shell whoami)
target := main
latex := pdflatex
bibtex := bibtex

.PHONY: default
default: all 

.PHONY: all
all:
	$(MAKE) checkbib $(target).pdf cleanmost

checkbib: 
	sh ./get_bib.sh

%.pdf: %.tex $(wildcard *.tex) 
	$(latex) $<
	$(bibtex) $*
	$(latex) $<
	$(latex) $<

one:
	$(latex) $(target).tex

bib:
	$(bibtex) $(target)

.PHONY: clean
clean:
	make cleanmost
	rm -f $(patsubst %,%.fls,$(target)) \
	$(patsubst %,%.out,$(target)) \
	$(patsubst %,%.fdb_latexmk,$(target)) \
	$(patsubst %,%.synctex*,$(target)) \
	$(patsubst %,%.synctex.gz,$(target))

.PHONY: cleanmost
cleanmost:
	rm -f *~ *.bak \
	$(patsubst %,%.dvi,$(target)) \
	$(patsubst %,%.log,$(target)) \
	$(patsubst %,%.aux,$(target)) \
	$(patsubst %,%.bbl,$(target)) \
	$(patsubst %,%.blg,$(target)) \
	$(patsubst %,%.lox,$(target)) \
	$(patsubst %,%.upa,$(target)) \
	$(patsubst %,%.upb,$(target)) \
	$(patsubst %,%.xcp,$(target))

.PHONY: cleanall
cleanall:
	make clean
	rm -f $(patsubst %,%.pdf,$(target))

.PHONY: copy
copy:
#ifeq ($(whoami),manos)
#	rsync -a top.pdf <someshere>
#endif




==> biblio_something.tex <==
%\bibliography{../../../../Dropbox/W-Lab/Bibliography-Mendeley/library, bibl}
%\bibliography{../../Dropbox/Professional/Professorship/W-Lab/Bibliography-Mendeley/library,bibl,tmp/matt_bittex}
\bibliography{../mendeley-library/library,bibl,tmp/matt_bittex}

==> old-text/abstract.tex <==

% \begin{abstract}
    Almost sorted data can be termed as a property of "near-sortedness" where data has some amount pre-existing order and nearly perfect. 
    arious metrics exist that identify the near-sortedness in a data collection and capture useful information about the dataset in different magnitudes. 
    Quantifying "near-sortedness" is done on a case-by-case basis and is dependent on the information captured specific to a particular application. 
    Sorting algorithms use ordering in datasets as edge-cases while proving efficiency while adaptive sorting algorithms work towards achieving a 
    middle ground between both ends. Common indexes like $B+$-trees and $B^\epsilon$-trees exhibit similar performances for completely ordered data 
    as well as un-ordered data for both inserts and reads. However, bulk loading achieves a much better performance by utilizing the order prevalent 
    in the dataset and avoiding unnecessary tree-based computations. Near-sortedness though to a particular order is expected to perform close to the 
    bulk-loading, does not follow expectations and exhibits general traits with the indexes. Hence, there is a need to leverage the near-ordering in 
    data to amortize the computational costs with inserts in popular tree-based indexes and enhance efficiency. 
% \end{abstract}

==> old-text/analysis.tex <==
\subsection{Metrics}
The trends of different metrics with varying $k$ is shown in Figure \ref{fig:metric_trends}). The $x-$axis on all images is the varying noise 
$\%$ whereas the $y-$axis is the value corresponding to a metric. Each point on the graph denotes a particular near-sorted dataset collection 
corresponding to a particular $(k,l)$ value as defined in the graphs.

Notice that Figure \ref{fig:metric_trends_runs} and \ref{fig:metric_trends_exchanges} show trends similar to Figures 
\ref{fig:metric_trends_inversions} and \ref{fig:metric_trends_enc_lists}, however the difference in the maximum and minimum values are very 
little in the former group. This can be extended to say that runs and exchanges are easy metrics to quantify near-sortedness, but do not 
capture enough information that offers deeper insights into the data collection. This is not the case with Figures \ref{fig:metric_trends_inversions} 
and \ref{fig:metric_trends_enc_lists} where there is significant difference between data points on the graph meaning they increase significantly as 
noise increases, thus proving themselves to be useful metrics. In case of Figures \ref{fig:metric_trends_las} and \ref{fig:metric_trends_rem}, there 
is no specific pattern that is followed with increasing noise - this is expected since the $las$ and $rem$ are both not particularly assigned with the 
$(k,l)$ parameters, since elements that meet upto $k$ are picked randomly from a window specified by $l$. 

As discussed previously, metrics like Runs, Inversions, exchanges and encroaching lists have their own disadvantages. Longest Ascending Subsequence 
and $Rem$ are void of those disadvantages but do not show a concrete trend with increasing noise, hence making them difficult to comprehend and predict 
the traits. The intuition is that both these metrics are dependent on the distribution density of scrambled elements which was not included in the 
experimental parameters and is out of scope of this project (due to time constraints). The $(k,l)-$parameter on the other hand captures as much information 
as possible with the number of elements out of order and shuffle window, effectively making itself a combination of all other metrics: 
    \begin{itemize}
        \item The parameter $k$ that signifies the out of order elements is close to what is captured by $Inv(X)$ or $Exc(X)$.
                Increase in $k$ means more elements are out of place and this in-turn increases the no. of inversions or exchanges.  
        \item The parameter $l$ offers a window within which elements can be shuffled. An increase in $k$ and $l$ should increase the $Rem(X)$
                and subsequently decrease the $Las(X)$ since there is a greater possibility of shuffling elements that are further away. 
    \end{itemize}

    \begin{figure}[!htb]
        \centering
        \begin{subfigure}[b]{0.225\textwidth}
            \centering
            \includegraphics[scale=0.17]{images/runs.png}
            \caption{Runs}
            \label{fig:metric_trends_runs}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.225\textwidth}
            \centering
            \includegraphics[scale=0.17]{images/inversions.png}
            \caption{Inversions}
            \label{fig:metric_trends_inversions}
        \end{subfigure}

        \vskip\baselineskip

        \begin{subfigure}[b]{0.225\textwidth}
            \centering
            \includegraphics[scale=0.17]{images/exchanges.png}
            \caption{Exchanges}
            \label{fig:metric_trends_exchanges}
        \end{subfigure}
        \quad
        \begin{subfigure}[b]{0.225\textwidth}
            \centering
            \includegraphics[scale=0.17]{images/encroaching_lists.png}
            \caption{Encroaching Lists}
            \label{fig:metric_trends_enc_lists}
        \end{subfigure}

        \vskip\baselineskip

        \begin{subfigure}[b]{0.225\textwidth}
            \centering
            \includegraphics[scale=0.17]{images/las.png}
            \caption{Longest Asc. Subsequence}
            \label{fig:metric_trends_las}
        \end{subfigure}
        \quad
        \begin{subfigure}[b]{0.225\textwidth}
            \centering
            \includegraphics[scale=0.17]{images/rem.png}
            \caption{Rem}
            \label{fig:metric_trends_rem}
        \end{subfigure}
    \caption{Different Metrics with varying $k$ \%}
    \label{fig:metric_trends}
    \end{figure}

\subsection{Sorting}
As mentioned earlier, the differently sorted collections were tested with popular 
in-memory algorithms like Quicksort and Insertion Sort and an adaptive sorting algorithm proposed by \cite{Ben-Moshe2011}.
The results of experiments on the different sorting algorithms tested 
on 1 Million elements with multiple degrees of \textit{near-sortedness} is 
shown in Figure \ref{fig:combined_sorting}).

    \subsubsection{Sequential Scan}
    Sequential scan is a basic run over the data without any computations. 
    It remains constant irrespective of noise levels. 

    \subsubsection{Quicksort}
    Quicksort produces an average-case runtime of $O(nlogn)$ and a worst-case
    runtime of $O(n^2)$. We observe a worst-case runtime with Quicksort when the collection is 
    completely ordered. Figure \ref{fig:workloads})(a) shows a very large execution time for Quicksort (outside the scale in the graph) when all 
    elements are in place, and this value decreases as increase the noise in the data. 

    \subsubsection{Insertion Sort}
    Insertion sort is a very effective algorithm that would finish execution in 
    linear time ($O(n)$) if the collection is sorted, but has an average and worst
    case quadratic runtime $O(n^2)$. Our expectation was that insertion sort should 
    work reasonably well with \textit{near-sorted} data, before exhibiting its average 
    and worst case performance as noise increases. A good trend is seen in Figure
    \ref{fig:workloads})(a), where insertion sort has quick runtime for completely ordered
    data and increases its runtime with increasing noise levels. Figure 
    \ref{fig:workloads})(b) shows the graph for insertion sort starting at a higher execution 
    time and subsequently moving out of the graph scale which is mainly attributed to the 
    $l \%$, or the increase in shuffle window. For this same reason, insertion sort trends are 
    hidden from subsequent plots as they were outside the general scale of the graph. 

    \subsubsection{Adaptive Algorithm}
    The adaptive algorithm looks the best bet for sorting a family of differently 
    sorted collections since it shows similar trends for different shuffle windows 
    ($l \%$) and also does not exhibit steep increase in runtime with increasing 
    noise. That is, it works on both ends of the spectrum: similar runtime as 
    insertion sort that works best for completely ordered data, and comparable runtime 
    with Quicksort that works best for completely random data where it increases slowly as the noise in the data increases. 
    
    \begin{figure}[!htb]
        \centering
        \begin{subfigure}{0.225\textwidth}
            \centering
            \includegraphics[scale=0.17]{images/sorting/combined/l-1.png}
            \caption{1M Elements with $l = 1\%$}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.225\textwidth}
            \centering
            \includegraphics[scale=0.17]{images/sorting/combined/l-10.png}
            \caption{1M Elements with $l = 10\%$}
        \end{subfigure}
        
        \vskip\baselineskip
    
        \begin{subfigure}{0.225\textwidth}
            \centering
            \includegraphics[scale=0.17]{images/sorting/combined/l-30.png}
            \caption{1M Elements with $l = 30\%$}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.225\textwidth}
            \centering
            \includegraphics[scale=0.17]{images/sorting/combined/l-50.png}
            \caption{1M Elements with $l = 50\%$}
        \end{subfigure}
        
    \caption{Runtime of in-memory sorting algorithms on family of differently sorted collections
     of 1 Million Integers with varying $k$ \%  and $l$ \% )}
    \label{fig:combined_sorting_old}
    \end{figure}

\subsection{Data Structures and Indexes}
The performance of $B+$-trees and $B^\epsilon$-trees with varying noise for inserts and reads is shown in Figure \ref{fig:data_struct}. 
For reads (Figure \ref{fig:data_struct_read}), we can see that both indexes show similar execution times even if we increase the noise levels 
in the data, and this is expected as queries are independent of such noise levels since query is executed after adding all the elements to the index. 
The interesting results are obtained for the insertion costs, where a trend similar to reads is observed (Figure \ref{fig:data_struct_insert} with 
a red and blue trend-line). From a worst-case perspective where the data is completely scrambled, this is a win-scenario since the index does the 
same amount of work as with an already ordered dataset. However, from the best-case perspective or near-best case scenario in terms of near-sorted 
data, more work is being done without accounting for pre-existing order in the data. Near-sortedness should be leveraged in case of inserts to account 
for the existing order and subsequently adjust the insert mechanism to perform less work. When the $B+$-tree is bulk-loaded, we see a significant decrease 
in insertion cost since it is void of internal splits or leaf splits (these account for added time in case of normal inserts). Hence, an ideal situation 
would be that the index performs the least work for completely ordered data and its cost is closer to that of bulk-loading, and increases the insertion 
cost as the data becomes more scrambled or unordered where the insertion cost is at the current rate at maximum. The constant performance trend is 
visible for both the indexes, but it is also observed that the $B^\epsilon$-tree insert cost is much less than that of the $B+$-tree due to its buffer. 
Thus, the buffer plays a significant role to amortize the read costs in the tree-based indexes and adjusting the flush threshold adaptive of near-sortedness 
in data could be an interesting direction for future work where efforts could be made to reduce the cost for inserts for near-sorted data. 

    \begin{figure}[!htb]
        \centering
        \begin{subfigure}{0.45\textwidth}
            \centering
            \includegraphics[scale=0.4, width=\textwidth]{images/data_struct_read.png}
            \caption{Reads (Existing Query)}
            \label{fig:data_struct_read}
        \end{subfigure}
        
        \vskip\baselineskip
    
        \begin{subfigure}{0.45\textwidth}
            \centering
            \includegraphics[scale=0.4, width=\textwidth]{images/data_struct_insert.png}
            \caption{Inserts}
            \label{fig:data_struct_insert}
        \end{subfigure}
       
    \caption{Execution Time of $B+$-trees and $B^\epsilon$-trees with node size of $4096$ bytes and Data of $L=10\%$}
    \label{fig:data_struct}
    \end{figure}

\subsection{Zonemaps}
    The performance of zonemaps with varying noise $\%$ and also varying the number of zones is shown in Figures \ref{fig:zonemaps_noise} and 
    \ref{fig:zonemaps_zones} respectively. In a range query of $50000$ elements, if the data is completely sorted and each zone has $1000$ elements, 
    then approximately $50$ zones need to be scanned. However, if some noise exists in the data, this might vary and would probably increase as more 
    zones would have elements that are out-of-place from their respective zones (in case of sorted order). Thus, it was expected that the query time 
    would increase. However, the results did not show any specific pattern, as shown in Table \ref{tab:zonemaps_noise_table}. This can be attributed 
    to the varied distribution of scrambled elements in our data collection. It is possible that for a specific noise level, the density of scrambled 
    elements is more in one particular area of the dataset, thereby only a few zones might have such out-of-place elements in higher density. 
    Our range query in such cases would capture lesser zones than expected and would have an execution time that is lower than the expectations. 
    Thus, it is not practical to extend the idea of increased noise means increased execution time in this case. One such way to fix such an issue would 
    be to specify a distribution for the noise in the dataset, but it is out of the scope of this project (due to time constraints).
    
    The performance of zonemaps with varying zones is shown in Figure \ref{fig:zonemaps_zones}. As we increase the number of zones, more zones need to be 
    scanned for a range query, hence the execution time should increase. The results obtained are consistent with such expectations. Figure \ref{fig:zonemaps_zones} 
    marks an increasing trend in execution time as we increase the number of zones for a particular dataset (marked by a red line). 
    
    Additionally, the minimum and maximum value in every zone was also plotted as shown in Figure \ref{fig:zonemap_visuals} to visualize the scrambling 
    in every zone. Figure \ref{fig:zonemap_vis_0} shows how the minimum and maximum would line up for completely ordered data - showing a linear trend. 
    As we increase the noise, we see that the minimum and maximum move away from the perfect linear trend to show spikes in the graph in Figures \ref{fig:zonemap_vis_25}, 
    \ref{fig:zonemap_vis_50} and \ref{fig:zonemap_vis_100}. The spikes are a result of misplaced elements in zones that they are not supposed to be present in, 
    if the data is completely ordered. The spikes are also minor, since the dataset had an $l\% = 10$, so the shuffling was $\pm 10\%$ from their actual position. 
    If this percentage is increased, the spikes for minimum and maximum would be greater in magnitude. 
    
    \begin{table}[!h]
    	\centering
    	\begin{tabular}{|c |c c |}
            \hline\hline
            Noise $\%$ & Zonemap ($\mu$s) & Linear Search ($\mu$s)  \\
            \hline
            0   & 2222 & 6102 \\
            25  & 2093 & 6114 \\
            50  & 2121 & 6148 \\
            100 & 2063 & 6097 \\
    	    \hline
    	\end{tabular}
    	\caption{Query Performance (Zonemap and Linear Search) with Varying Noise for 1 Million elements in 1000 Zones}
    	\label{tab:zonemaps_noise_table}
    \end{table}
    
    \begin{figure}[!b]
        \centering
        \begin{subfigure}{0.45\textwidth}
            \centering
            \includegraphics[scale=0.25, width=0.8\textwidth]{images/zonemaps_noise.png}
            \caption{Varying Noise}
            \label{fig:zonemaps_noise}
        \end{subfigure}
       
        \vskip\baselineskip
    
        \begin{subfigure}{0.45\textwidth}
            \centering
            \includegraphics[scale=0.25, width=0.8\textwidth]{images/zonemaps_zones.png}
            \caption{Varying Number of Zones}
            \label{fig:zonemaps_zones}
        \end{subfigure}
    \caption{Query Performance of Zonemaps and Linear Search for 1 Million Elements}
    \label{fig:zonemaps_performance}
    \end{figure}
    
    \begin{figure}[!b]
        \centering
        \begin{subfigure}{0.225\textwidth}
            \centering
            \includegraphics[scale=0.17]{images/zones-0k.png}
            \caption{$k=0\%$}
            \label{fig:zonemap_vis_0}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.225\textwidth}
            \centering
            \includegraphics[scale=0.17]{images/zones-25k.png}
            \caption{$k=25\%$}
            \label{fig:zonemap_vis_25}
        \end{subfigure}
        
        \vskip\baselineskip
    
        \begin{subfigure}{0.225\textwidth}
            \centering
            \includegraphics[scale=0.17]{images/zones-50k.png}
            \caption{$k=50\%$}
            \label{fig:zonemap_vis_50}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.225\textwidth}
            \centering
            \includegraphics[scale=0.17]{images/zones-100k.png}
            \caption{$k=100\%$}
            \label{fig:zonemap_vis_100}
        \end{subfigure}
        
    \caption{Overlap in Minimum and Maxiumum element in every zone for $1000$ zones with $l=10\%$}
    \label{fig:zonemap_visuals}
    \end{figure}
 

==> old-text/approach.tex <==
\subsection{Solution Design}
\subsubsection{Near Sortedness with Algorithms and Indexes}
\begin{enumerate}
    \item A family of differently sorted collections is created with 1 Million elements (each are positive integers), with different $k$ and $l$ parameters as percentage of the total elements in the dataset. Duplication is avoided as much as possible. 
    
    \item The family of differently sorted collections are then tested with in-memory sorting algorithms - Insertion Sort and Quicksort, as well as adaptive algorithm described by \cite{Ben-Moshe2011}. The execution time is measured.
    
    \item The differently sorted collections is also tested with two popular indexes - $B$-trees and $B+$-trees, and the insertion and query time (existing queries) is measured. 
    
    \item The data collections are also tested with a naive implementation of zonemaps (discussed further in Section \ref{sec:zonemaps_design}). The query time for a range query and the minimum and maximum values in every zone is also noted to study the overlaps in the zones due to varying degree of near-sortedness. 
\end{enumerate}


==> old-text/background.tex <==
\subsection{Measures of Pre-sortedness or Near-Sortedness}
\label{sec:presortedness_metrics}
    Assume $X = \langle x_1, x_2, \ldots, x_n \rangle$ be the input of length $n$ to be sorted. The following metrics 
    quantify the varying degree of sortedness in the given input. 
    
    \subsubsection{Inversions (Inv)}
    Manilla \cite{Mannila1985} described inversions as the number of pairs in incorrect order. Assuming ascending order, 
    inversions $Inv(X) = | { (i,j) | 1 \leq i < j \leq n, x_i > x_j } |$. Also, $ 0 \leq Inv(X) \leq n(n-1)/2 $ for all $X$, 
    with the smallest value fo $Inv(X)$ occuring in case of a completely sorted list and the largest value in case of a list 
    in the opposite order (descending). Though widely studied and used, it has a major drawback that inputs of type 
    $(n+1, n+2, \ldots, 2n, 1, 2, \ldots, n)$ yield a quadratic number of inversions, though they are almost in order and can 
    be sorted easily by dividing the list into two equal halves and merging the first after the second half. 

    \subsubsection{Runs}
    Runs can be simplified as the number of contiguous increasing subsequences of $X$ and \cite{Mannila1985} defines 
    $Runs(X) = | \{ i | 1 \leq i < n $, $a_{i+1} < a_i\}$ $ | + 1$, where $Runs(X) = 1$ or $n$ when the list is already sorted or 
    is in reverse order respectively. This measure also comes with a drawback that local disorder  produces a lot of runs, 
    though the sequence can be easily sorted through bubblesort. 

    \subsubsection{Longest Ascending Subsequence (LAS) and Rem}
    The longest ascending subsequence can be visualized as an extension of the previous metric (Runs), signifying the length 
    of the longest run of $X$. \cite{Mannila1985} defines Longest Ascending Subsequence as 
    $Las(X) = max\{ t | \exists i(1), \ldots, i(t), 1 \leq i(1) < \ldots < i(t) \leq n, x_{i(1)} < \ldots < x_{i(t)} \}$ and 
    $Rem(X) = n - Las(X)$ that signifies the number of elements to be removed from X to achieve complete order in the list. 
    $Rem(X) = 0$ or $n-1$ based on whether the list is sorted or in reverse order. 

    \subsubsection{Exchanges (Exc)}
    Exchanges are defined by \cite{Mannila1985} as the smallest number of exchanges of arbitrary elements needed to bring $X$
    into ascending order. So, $Exc(X) = 0$ for a completely ordered list and $Exc(X) \leq inv(X)$ for all $X$. The upper bound 
    of exchanges takes into the number of cycles in the permutation ${1, \ldots, n}$ for $X$. Every permutation has at least 
    one cycle so $Exc(X) \leq n - 1$ for all $X$. 

    \subsubsection{Enchroaching Lists (EL)}
    Consider an ordered list $l$, with $head(l)$ being the smallest element in $l$ and $tail(l)$ the largest element in $l$. 
    An \textit{encroaching list} set is an ordered set of \textit{ordered lists} $l_1, \ldots l_m$, such that 
    $head(l_i) \leq head(l_{i+1})$ and $tail(l_i) \geq tail(l_{i+1})$ for $1 \leq i < m$. The size of this list set $m$ is 
    dependent on the measure of pre-sortedness and thus can be used to quantify the degree of sortedness of data. This size 
    increases with increasing randomness in data \cite{Skiena1988}. 
    
    \subsubsection{(k,l)- nearly sorted}
    Ben-Moshe defined nearly sorted relations with respect to two parameters $k$ and $l$ \cite{Ben-Moshe2011}. The number of 
    unordered elements where captured by $k$ and the window through which elements could be shuffled within the domain was 
    captured by $l$. On a simpler note, $l$ tells us how rough is the sorting or how far elements can be from their actual 
    ordered position, and $k$ tells us how many such elements are out of place.

    
\subsection{Sorting Algorithms}
    \subsubsection{Quicksort}
    Quicksort is a divide and conquer algorithm that picks a pivot element around which the given array/collection is 
    partitioned around. The pivot can be picked in many ways - first element, last element, random element or median element. 
    The algorithm has a runtime of $O(nlogn)$ on the average case and has a worst case run-time of $O(n^2)$, when either the 
    first or last element is chosen as the pivot and the array is already sorted \cite{Quicksort}. 
    
    \subsubsection{Insertion Sort}
    Insertion sort is a simple sorting algorithm that works similar to the way a hand of playing cards are sorted. It has 
    a time complexity of $O(n^2)$ on the average and worst case but the best case complexity is $O(n)$ when the array/collection 
    is already sorted \cite{InsertionSort}. 
    
    \subsubsection{Adaptive Sorting Algorithm - BenMoshe}
    The adaptive sorting algorithm described in \cite{Ben-Moshe2011} sorts a $(k,l)$-nearly sorted collection in at most two 
    sequential passes. The first pass is similar to the Replacement-Selection Algorithm where it collects the set of misplaced 
    entries. The subsequent pass involves placing the misplaced/collected tuples in their correct locations (merge phase). 
    The algorithm takes $O(nlog(k+l))$ computations, thus it is comparative to the Quicksort algorithm on the worst case. 

\subsection{$B+$ -Trees}
B+ Trees are an extension of B-trees that allow for (key,value) storage in a tree structure. 
A traditional B+-tree has one root, a number of internal nodes and leaf nodes (shown in Figure \ref{fig:b_plus_tree}). Unlike a B-tree, 
data pointers are only stored in the leaf nodes along with all key values as shown in figure. Each leaf node is also 
linked to its successor to provide ordered access. Key values of leaf nodes could also be part of 
internal nodes to act as a medium of control for querying records. The insertion and query (existing) cost for the 
$B+$-tree is $O(log_F (N))$, where $F$ is the fanout in the tree. 

\begin{figure}[!htb]
    \centering
    \includegraphics[scale=0.5, width=0.5\textwidth]{images/b_plus_tree.jpg}
    \vspace{-0.25in}
    \Description{$B+$-tree}
    \caption{Standard $B+$-tree}
    \vspace{-0.1in}
    \label{fig:b_plus_tree}
\end{figure}

\subsubsection{Bulk Loading}
When we have a large number of records, inserting them one-by-one is a slow process and hence the index can be bulk-loaded. 
For bulk-loading a $B+$-tree, it is required that the data be sorted and index entries for leaf pages are always entered 
into rightmost index page just above leaf level. Several internal computations of the tree and hence is much faster than 
regular inserts. The primary advantage of bulk loading is the fewer I/Os and sequential storing of the leaf nodes. 


\subsection{{$B^\epsilon$} -Trees}
A $B^\epsilon$-tree is a write-optimized data structure proposed by Brodal And Fagerberg \cite{Brodal2003} as B-trees with 
buffers (shown in Figure \ref{fig:b_epsilon_tree}). The buffer offers ability to improve the I/O bound for updates in the 
tree without sacrificing query performance. Every node in the tree has a buffer, where updates are delayed and propagated 
down whenever there is a buffer overflow. Elements from the buffer of this node are then moved to the buffer of the child node, 
similar to a buffer tree. The insert and read cost are similar to the $B+$-tree but are a factor of $\epsilon$. On a general 
case, the insertion cost is $O(\frac{log_B (N)}{\epsilon B^{1-\epsilon}})$ and the read cost is $O(\frac{log_B (N)}{\epsilon})$. 
If $\epsilon = \frac{1}{2}$, then the cost of insertion becomes $O(\frac{log_B (N))}{\sqrt{B}}$ and the read cost becomes $O(log_B (N))$. 

\begin{figure}[!htb]
    \centering
    \includegraphics[scale=0.45]{images/bepsilon_tree.png}
    \Description{$B^\epsilon$-tree}
    \caption{$B^\epsilon$-tree}
    \label{fig:b_epsilon_tree}
\end{figure} 

\subsection{Zonemaps}
Zone-Maps in database are structures similar to indexes that allow pruning disk blocks and potentially full partitions of a 
partitioned table based on predicates on the table columns. They divide the collection into partitions called \textit{zones}, 
and store the min and max value for every \textit{zone}. A zone is a set of a contiguous data blocks on disk. Zone maps can 
be used with or without attribute clustering. It stores information per zone instead of per row, hence it is much more compact 
than an index \cite{Zonemaps}.


==> old-text/benchmark.tex <==
Assume a set of tuples (array of elements for simplicity) $X$. A nearly sorted collection $f$ can be defined as $f = X <k,l>$ 
where $k$ is the number of out-of-order elements in $X$ and $l$ is the shuffle window (maximum displacement from its actual position), 
both as a percentage of $n$ - the total number of elements in $X$. 

A family $\mathcal{F}$ of differently sorted collections can be defined as follows: 
    \begin{equation}
        \mathcal{F} = \{f_1, f_2, \ldots, f_n | f_i = X <k_i,l_l> \}
    \end{equation}
or just simply saying a family of differently sorted collections can each be defined by a set of tuples that are arranged in some 
order specified by its own $k,l$ respectively. These collections can also be called near-sorted with respect to $k,l$ or just $(k,l)$
-nearly sorted collections. 

A metric $M$ pertaining to a $(k,l)$-nearly-sorted collection can be defined as the number of occurrences of a pattern/trait for 
the particular $(k,l)$-nearly sorted collections. So, if we have $p$ metrics, then each $M_j = Occurence_{M_j}(X<k,l>)$, i.e. each 
metric corresponds to its occurence for a specific nearly sorted collection.


While comparing two different metrics, we can say metric $M_1 > M_2$ if $|M_1| > |M_2|$, where each $M_1,M_2$ can be written as 
$|M_j| = |Occurence_{M_{j}}(X<k_{i+1}, l_{i+1})$ $-$ $Occurence_{M_{j}}(X<k_i,l_i>)|$, i.e. each metric is defined by the absolute 
value of difference in their occurrences for successive/subsequent data collections and each collection is defined by its own $k,l$. 
Simply put, we can say $M_1 > M_2$ if the former captures more information than the latter. 

Let $t_1$ be the execution time for a sorting algorithm $A_1$ and $t_2$ be the execution time for sorting algorithm $A_2$. Then:
    \begin{equation}
        t_1 < t_2 \Rightarrow A_1 > A_2
    \end{equation}
To simplify, if $t_1$ is less than $t_2$, algorithm $A_1$ is better than $A_2$. A similar argument can be extended to even data 
structures. Let $z_1$ be the execution time for a data structure/index $D_1$ and let $z_2$ be the execution time for a data 
structure/index $D_2$. Then, for an operation $O$: 
    \begin{equation}
        z_1 < z_2 \Rightarrow D_1 > D_2
    \end{equation}
Or we can simply say that for an operation $O$ (like insert, query, etc.), if the execution time for $z_1$ is less than $z_2$, 
structure $D_1$ is better than $D_2$.

\textbf{Note}: These are mathematical expressions that drive the explanations given in the analysis section. The latter sections 
of this paper uses simple terms to distinguish between collections, algorithms and indexes rather than mathematical terms to 
enhance readability of the paper.  

==> old-text/conclusion.tex <==
Pre-sortedness is a property of existing order in a data collection and near-sortedness can be simplified as a measure of pre-sortedness 
by itself, where the data collection is close to a particular order with respect to a particular attribute. Various metrics for 
near-sortedness/pre-sortedness exist like runs, inversions, exchanges, longest ascending subsequences and rem, where a few capture useful 
information between different datasets whereas others do not show much change and hence do not capture enough detail.  A family of differently 
sorted collections uses the $(k,l)$ parameters to quantify near-sortedness. These differently sorted collections when tested with in-memory 
sorting algorithms and an adaptive sorting algorithm showed expected behavior where Quicksort performed worst for completely ordered data 
whereas insertion sort performed worst for unordered data. Adaptive sort achieves a balanced performance between both extremes by matching 
performance of insertion sort for ordered and nearly-ordered data and slowly increasing its run-time comparable to quick-sort on the other 
end of the spectrum. Tree-based indexes show a constant performance for both reads and inserts even with varying level of sortedness, 
without accounting for existing order prevalent in the data collection. Bulk loading of $B+$-trees performs the best for inserts and 
the buffer in the $B^\epsilon$-tree reduces the cost of inserts to an extent, thus an optimized buffered approach for inserts would 
be the right direction to amortize the costs. Query execution time with zonemaps increases due to noise in the data but does not show a 
specific trend due to the distribution density of out-of-order elements. Increase in the number of zones however increases the query execution time. 

\subsection{Future Work}

There are several modifications that could be made to the existing solution design to make it more robust towards the benchmark expectations, 
which unfortunately could not be done due to time constraints. In creating the family of differently sorted data, a visualization of the 
distribution for noise in the dataset would further validate the current interpretations for the metrics and also provide other key insights. 
It would also be ideal to set the distribution density of scrambling as a parameter while creating the data so that it would be more useful for 
testing with the algorithms (especially analyzing how the distrubution/density affects the performance of the algorithms), indexes and zonemaps. 
As for indexes, there are minor differences in implementation of both indexes, which might account for deviations in expected performance values 
for reads and inserts in both indexes, though they maintain the high-level motive. Ideally, both implementations should be integrated into the 
same framework to provide a robust comparison, which is time-intensive and is left for future work. For the zonemaps, as mentioned earlier, 
adding the distribution density would offer key insights into their performance with varying noise and this could be a good project to be 
pursued/studied further. 

Currently, the authors are working on techniques that can modify the buffer with $B^\epsilon$-trees and also adding an additional buffer 
for the $B+$-trees that can capture near-sortedness in the data and can perform semi-bulk-loading (like range inserts for a batch of elements 
flushed from the buffer). The key areas for exploration in this project includes identifying the flush threshold such that it captures the 
near-sortedness in data and optimizing the inserts such that the number of internal node and leaf splits are minimized while inserting 
near-sorted data. This would essentially lead to the $OSM$-Tree for the $B$-tree case and can be extended to the $LSM$-Tree.


==> old-text/evaluation.tex <==
\subsection{Setup}
The experiments were done in a linux server with 80-Cores and an 2.10GHZ Intel(R) Xeon(R) Gold 6230 processor
with 383GB of system memory and L1 (d,i) cache of (32K,32K), L2 Cache of 1024K and L3 cache of 28160K. 
All experiments were conducted on a data set size (length) of 1 Million elements.

\subsection{Workload}
To generate a family of differently sorted collections, we used two parameters $k$ 
and $l$, where the former specified the number of elements to be shuffled and the 
latter specified the window through the elements can be shuffled. The differently 
sorted collections are shown in Figure  \ref{fig:workloads}). We can simplify $k$ as the number of 
distortions to a straight line and $l$ can be the magnitude of the distortions/spikes. The magnitude of 
spikes varies the $l\%$ changes as seen in the figure for larger values for $l\% = 10,30$. This is because 
$l$ represents the shuffle window, so a larger $l$ means that it can pick an element farther away from its 
in-place position while generating the noise. 

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.15\textwidth}
        \centering
        \includegraphics[scale=0.12]{images/workloads/5k-1l.png}
        \caption{5\% $k$ - 1\% $l$}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.15\textwidth}
        \centering
        \includegraphics[scale=0.12]{images/workloads/25k-1l.png}
        \caption{25\% $k$ - 1\% $l$}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.15\textwidth}
        \centering
        \includegraphics[scale=0.12]{images/workloads/70k-1l.png}
        \caption{70\% $k$ - 1\% $l$}
    \end{subfigure}
    \vskip\baselineskip

    \begin{subfigure}[b]{0.15\textwidth}
        \centering
        \includegraphics[scale=0.12]{images/workloads/0k-10l.png}
        \caption{0\% $k$ - 10\% $l$}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.15\textwidth}
        \centering
        \includegraphics[scale=0.12]{images/workloads/5k-10l.png}
        \caption{5\% $k$ - 10\% $l$}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.15\textwidth}
        \centering
        \includegraphics[scale=0.12]{images/workloads/50k-10l.png}
        \caption{50\% $k$ - 10\% $l$}
    \end{subfigure}
    \vskip\baselineskip

    \begin{subfigure}[b]{0.15\textwidth}
        \centering
        \includegraphics[scale=0.12]{images/workloads/0k-30l.png}
        \caption{0\% $k$ - 30\% $l$}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.15\textwidth}
        \centering
        \includegraphics[scale=0.12]{images/workloads/5k-30l.png}
        \caption{5\% $k$ - 30\% $l$}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.15\textwidth}
        \centering
        \includegraphics[scale=0.12]{images/workloads/50k-30l.png}
        \caption{50\% $k$ - 30\% $l$}
    \end{subfigure}
\caption{Workloads with varying $k$ \% (out of order elements) and $l$ \% (shuffle window)}
\label{fig:workloads}
\end{figure}

\subsection{$B+$-trees and $B^\epsilon$-trees}
Both $B+$-trees and $B^\epsilon$-trees are configured with a node size of $4096$ bytes. The $B+$-tree uses
 a standard $STX$ implementation from \cite{BTree}, whereas the $B^\epsilon$-tree is modelled from an 
 implementation by \cite{BepsilonTree} and combined with a few textbook design solutions found in \cite{bender2015}. 
 Further, the buffer size and other specifics for the $B^\epsilon$-tree were configured as follows: 
\begin{itemize}
    \item Leaf Size $= 4088$ bytes
    \item Buffer Size $= 4025$ bytes 
    \item Pivot Size $= 63$ 
    \item Leaf Flush Threshold $= 256$
    \item Number of children per node $ = 63$
\end{itemize}
Further, the bulk-loading time was also measured for the $B+$-tree to compare with general inserts. 

\subsection{Zonemaps}
\label{sec:zonemaps_design}
A na\"ive implementation of zonemaps was used to study its effect on partitioning near-sorted data. Each zone 
has its own $zone\_id$, $max\_element$, $min\_element$ and a vector of $<elements>$ placed in the zone. Since we 
are dealing with all data only placed in memory, the zonemaps are treated as an array/vector of zones in this 
implementation. The following experiments were conducted: \begin{enumerate}
    \item Effect of varying noise in data while querying from zonemaps: By default the data of 1 Million elements 
    were divided into $1000$ zones in a sequential manner, followed by executing $100$ range queries and measuring 
    the execution time. Each query searched for $\approx 50000$ elements within the domain.
    
    \item Effect of varying number of zones: By using a specific data collection with $25\%$ 
    noise ($K = 25\%, L = 10\%$), $100$ range queries were executed for four different number of zones - $100, 1000, 5000, 10000$ 
    and the execution time was calculated. Each query searched for $\approx 50000$ elements within the domain.
\end{enumerate}

The experiments were also conducted with point-queries but produced inconsistent results attributed to the fact that 
the query was chosen to be a random number within the domain. It was likely that few trials chose numbers closer to 
the first zone or second zone whereas a few were in the latter zones. A range query however fetches all values/ number 
of entries in the zonemap within a given range so covers multiple zones, and hence produced better results. 
\section{New old evaluation}
%\begin{figure}[!htb]
%    \centering
%    \includegraphics[width=\columnwidth]{images/vary_buffer/Inserts_vary_buffer.pdf}
%    \caption{}
%    \label{fig:vary_buffer_ins}
%\end{figure}
%
%\begin{figure}[!htb]
%    \centering
%    \includegraphics[width=\columnwidth]{images/vary_buffer/Lookups_vary_buffer.pdf}
%    \caption{}
%    \label{fig:vary_buffer_queries}
%\end{figure}


% \begin{figure}[!thb]
%     \centering
%     \begin{subfigure}[b]{0.23\textwidth}
%         \centering
%         \includegraphics[scale=0.27]{images/vary_buffer/Inserts_vary_buffer.pdf}
%         \caption{$OSM+$\bplustree{} v/s.\bplustree{} Inserts}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.23\textwidth}
%         \centering
%         \includegraphics[scale=0.27]{images/vary_buffer/Lookups_vary_buffer.pdf}
%         \caption{$OSM+$\bepsilontree{} v/s. \bepsilontree{} Inserts}
%     \end{subfigure}
% \end{figure}

% \subsection{In-Memory Experiments}
% \Paragraph{\sysName{} is highly efficient for near-sorted inserts}
% Figure ~\ref{fig:osmgen3l} shows the performance of \sysName{} compared to 
% standard \bepsilontree{} and \bplustree{}. Clearly, the performance 
% of \sysName{} is highly efficient in case of inserts, and exhibits a gradual increase 
% in insert latency for both \bplustree{} and \bepsilontree{} configurations. Specifically, 
% for near-sorted workloads of noise levels ranging from $1-10\%$, \sysName{} takes only 
% a third of the time taken by the respective standard tree data structures. 
% Even in case of higher noise levels above $15\%$, \sysName{} is able to identify 
% sorted subsequences of data in a buffer cycle that are bulk loaded to reduce insert latency. 
% Out-of-order pages that are inserted through the root 
% have to traverse the entire tree in case of \bplustree{}, whereas \bepsilontree{} can batch these 
% inserts in every node's own buffer. Thus, \sysName{} $+$ \bepsilontree{} carries an advantage 
% even for higher noise levels.


% \begin{figure}[!thb]
%     \centering
%     \begin{subfigure}[b]{0.23\textwidth}
%         \centering
%         \includegraphics[scale=0.3]{images/gen/inserts-B+-OSM_1-L.png}
%         \caption{$OSM+$\bplustree{} v/s.\bplustree{} Inserts}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.23\textwidth}
%         \centering
%         \includegraphics[scale=0.3]{images/gen/inserts-BE-OSM_1-L.png}
%         \caption{$OSM+$\bepsilontree{} v/s. \bepsilontree{} Inserts}
%     \end{subfigure}
    
%     \vskip\baselineskip

%     \begin{subfigure}[b]{0.23\textwidth}
%         \centering
%         \includegraphics[scale=0.3]{images/gen/query-B+-OSM_1-L.png}
%         \caption{$OSM+$\bplustree{} v/s.\bplustree{} Point Lookups}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.23\textwidth}
%         \centering
%         \includegraphics[scale=0.3]{images/gen/query-BE-OSM_1-L.png}
%         \caption{$OSM+$\bepsilontree{} v/s. \bepsilontree{} Point Lookups}
%     \end{subfigure}
   
% \caption{Performance of \sysName{} with $1\%$ \pinBufName{} size 
% compared to \bplustree{} and \bepsilontree{} with $100\%$ memory allocation 
% in buffer pool cache}
% \label{fig:osmgen3l}
% \end{figure}


% \Paragraph{\sysName{} maintains a comparable performance with minor overhead for point queries}
% In case of point lookups, the \pinBufName{} adds an overhead to the regular lookup cost. 
% Our experiments indicate that the lookup latency of \sysName{} is less than $2\times$ that of the standard 
% \bplustree{} and \bepsilontree{}, when the size of \pinBufName{} is fixed at $1\%$ of the total data size.
% Figure ~\ref{fig:osmprofile} shows the performance breakdown of $5$ Million point queries on the 
% \sysName{}. Scanning the BF, and scanning the \emph{sorted} section of the \pinBufName{} with interpolation search 
% adds a negligble overhead, while scanning the tree is the most expensive due to the higher number of queries to the
% tree. Sequential scan has no involvement in the $0\%$-noise (completely sorted) dataset as expected, but impacts the 
% performance of further noise levels. Figure ~\ref{fig:seqprofile} shows the breakdown of sequential scans on the \emph{unsorted}
% section of the \pinBufName{}. We observe that the sequential search time is completely dominated by \emph{scanning within zones}, 
% which is essentially the sequential search performed on every page/zone once we filter the qualifying pages through the zone map.
% As the noise increases, there are more number of overlaps within the zones, hence more zones would qualify for the sequential scan. 
% This corresponds to the increase in point query time as the noise in the workload increases. 

% \begin{figure}[h!]
% 	\centering
%     \includegraphics[width=\columnwidth]{images/osmprofile.png}
%     \caption{Breakdown of $5M$ point queries on \sysName{} with $1\%$ \pinBufName{}
%     size and $100\%$ memory allocation in buffer pool cache.}
% \label{fig:osmprofile}
% \end{figure}

% \begin{figure}[h!]
% 	\centering
%     \includegraphics[width=\columnwidth]{images/seq-perf-profile.png}
%     \caption{Breakdown of sequential scan performance of \pinBufName{}}
% \label{fig:seqprofile}
% \end{figure} 

% \Paragraph{\sysName{} successfully captures sortedness within the buffer for reasonably 
% sorted data}
% Next, we analyze the performance of \sysName{} with different degrees of roughness in 
% sorting, or simply the $L$-window. The purpose of \pinBufName{} in the \sysName{}
% is to capture near-sortedness in the data. Higher $L$-windows imply more out-of-order 
% subsequences or pages, hence the insert time would move closer to the standard \bplustree{}. 
% Figure ~\ref{fig:osmlperf} shows the performance of $OSM+$\bplustree{} configuration against
% $L$-windows of $1\%, 10\%, 25\% \text{ and } 50\%$ for a fixed noise level. Clearly, for the lowest noise
% level of $1\%$, the $L$-window has a negligible impact on the insert latency because the 
% out-of-order elements are minuscule. However, larger noise levels coupled with larger $L$-windows 
% clearly impact the insert latency significantly. An $L$-window of $50\%$ implies a high degree 
% of roughness in sorting, which essentially results in maximum number of individual out-of-order 
% inserts to the tree. In such cases, we see that \sysName{} performs slightly worse than the standard 
% \bplustree{} due to the overhead added by the sorting attempts in \pinBufName{}. 

% \begin{figure}[htb]
%     \centering
%     \begin{subfigure}[b]{0.23\textwidth}
%         \centering
%         \includegraphics[scale=0.3]{images/l-windows/inserts-B+-OSM_1-p.png}
%         \caption{$1\%$ elements out of order}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.23\textwidth}
%         \centering
%         \includegraphics[scale=0.3]{images/l-windows/inserts-B+-OSM_10-p.png}
%         \caption{$10\%$ elements out of order}
%     \end{subfigure}
    
%     \vskip\baselineskip

%     \begin{subfigure}[b]{0.23\textwidth}
%         \centering
%         \includegraphics[scale=0.3]{images/l-windows/inserts-B+-OSM_25-p.png}
%         \caption{$25\%$ elements out of order}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.23\textwidth}
%         \centering
%         \includegraphics[scale=0.3]{images/l-windows/inserts-B+-OSM_50-p.png}
%         \caption{$50\%$ elements out of order}
%     \end{subfigure}
% \caption{Insert Performance of $OSM+$\bplustree{} with $1\%$ \pinBufName{} size 
% for varying degrees of roughness in sorting with $100\%$ memory allocation 
% in buffer pool cache}
% \label{fig:osmlperf}
% \end{figure}

% \Paragraph{Increasing size of \pinBufName{} reduces insert latency but adds significant overhead to 
% query performance}
% We further analyze the performance of \sysName{} by varying the size of the \pinBufName{}.
% Particularly, we see that while increasing the size of the \pinBufName{} improves insert performance 
% as it gives more opportunity to capture sortedness and bulk load more pages, it has a negative impact on 
% the query performance. This is mainly attributed to the increase in potential sequential scans on the unsorted parts of 
% the \pinBufName{}, which is highly expensive. From Eq. ~\eqref{eq:query_cost_buffer}, for $3000$ pages, the $\delta$ value (overhead) is $\approx$ 
% $4\times$ for \bepsilontree{} and $\approx 5.5\times$ for \bplustree{}, both of which are corroborated 
% by our experimental values shown in figures ~\ref{fig:osmbufsize3l05p}. 
% \begin{figure}[h!]
%     \centering
%     \begin{subfigure}[b]{0.23\textwidth}
%         \centering
%         \includegraphics[scale=0.3]{images/osmBuffer/inserts-B+-OSM_3-L-3-PBuf.png}
%         \caption{$OSM-$\bplustree{} v/s.\bplustree{} Inserts}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.23\textwidth}
%         \centering
%         \includegraphics[scale=0.3]{images/osmBuffer/inserts-BE-OSM_3-L-3-PBuf.png}
%         \caption{$OSM-$\bepsilontree{} v/s. \bepsilontree{} Inserts}
%     \end{subfigure}
    
%     \vskip\baselineskip

%     \begin{subfigure}[b]{0.23\textwidth}
%         \centering
%         \includegraphics[scale=0.3]{images/osmBuffer/query-B+-OSM_3-L-3-PBuf.png}
%         \caption{$OSM-$\bplustree{} v/s.\bplustree{} Point Lookups}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.23\textwidth}
%         \centering
%         \includegraphics[scale=0.3]{images/osmBuffer/query-BE-OSM_3-L-3-PBuf.png}
%         \caption{$OSM-$\bepsilontree{} v/s. \bepsilontree{} Point Lookups}
%     \end{subfigure}
   
% \caption{Performance of \sysName{} with $3\%$ \pinBufName{} size 
% compared to \bplustree{} and \bepsilontree{}}
% \label{fig:osmbufsize3l05p}
% \end{figure}

% % \begin{figure}[t!]
% %     \centering
% %     \begin{subfigure}[b]{0.23\textwidth}
% %         \centering
% %         \includegraphics[scale=0.3]{images/osmBuffer/inserts-B+-OSM_3-L-5-PBuf.png}
% %         \caption{$OSM-$\bplustree{} v/s.\bplustree{} Inserts}
% %     \end{subfigure}
% %     \hfill
% %     \begin{subfigure}[b]{0.23\textwidth}
% %         \centering
% %         \includegraphics[scale=0.3]{images/osmBuffer/inserts-BE-OSM_3-L-5-PBuf.png}
% %         \caption{$OSM-$\bepsilontree{} v/s. \bepsilontree{} Inserts}
% %     \end{subfigure}
    
% %     \vskip\baselineskip

% %     \begin{subfigure}[b]{0.23\textwidth}
% %         \centering
% %         \includegraphics[scale=0.3]{images/osmBuffer/query-B+-OSM_3-L-5-PBuf.png}
% %         \caption{$OSM+$\bplustree{} v/s.\bplustree{} Point Lookups}
% %     \end{subfigure}
% %     \hfill
% %     \begin{subfigure}[b]{0.23\textwidth}
% %         \centering
% %         \includegraphics[scale=0.3]{images/osmBuffer/query-BE-OSM_3-L-5-PBuf.png}
% %         \caption{$OSM+$\bepsilontree{} v/s. \bepsilontree{} Point Lookups}
% %     \end{subfigure}
   
% %     \caption{Performance of \sysName{} with $5\%$ \pinBufName{} size 
% %     compared to \bplustree{} and \bepsilontree{}}
% % \label{fig:osmbufsize3l5p}
% % \end{figure}

% \subsection{Disk-based Experiments}
% \Paragraph{\sysName{} offers significant speedups for near-sorted inserts}
% Figure ~\ref{fig:osmdisk10p_inserts} shows the performance speedup of $OSM-B^+$-tree compared to 
% standard \bplustree{}. In these experiments, we maintain a fixed size \pinBufName{} in \sysName{} at 
% $10,000$ pages ($0.5\%$ of the inserted data size). $OSM-B^+$-tree is highly efficient in case we ingest completely sorted data due to its 
% ability to bulkload the entire collection, offering upto an $8\times$ speedup as compared to a \bplustree{}. 
% When we introduce certain noise in the workload, the speedup decreases, yet, the
% \sysName{} is still significantly better compared to the standard \bplustree{}. Again, 
% the \pinBufName{} helps recognize sorted subsequences, sorts the remaining buffer if required and performs 
% bulkloading to reduce the ingestion cost. Even when inserting scrambled data with $K = 50\%$ and $L=50\%$, \sysName{} 
% offers a $2\times$ speedup over the \bplustree{}, showing that even a \pinBufName{} of size much smaller than the $L$-window 
% can still help \sysName{} outperform the \bplustree{} during ingestion. 
% % \Paragraph{\sysName{} maintains similar insert and read performance even with different memory 
% % allocations to the buffer pool cache}
% % Next, we analyze the performance of \sysName{} when writing to the disk. For this experiment, 
% % we reserve $10\%$ memory in the buffer pool and test with a workload constituting a $3\%$ $L$-window for different noise levels. 
% % The insert and point lookup latency for 
% % \sysName{} with $1\%$ \pinBufName{} are shown in figure ~\ref{fig:osmdisk10p}. As in the case 
% % of $100\%$ memory allocation in the buffer pool cache, \sysName{} is significantly faster for both 
% % \bplustree{} and \bepsilontree{} configurations. For point lookups, \sysName{} is at most $1.3\times$ the 
% % the performance of a standard \bplustree{}. \TODO{Analyze why performance of \sysName{} with \bepsilontree{} is faster 
% % for lower noise levels (intuition is early stopping with nodes mainly in memory)}.
% % near-sorted d
% \begin{figure}[!thb]
%     \centering
%     \begin{subfigure}[b]{0.23\textwidth}
%         \centering
%         \includegraphics[scale=0.3]{images/disk/osmBP_inserts.png}
%         \caption{$OSM-$\bplustree{} v/s.\bplustree{} Inserts}
%         \label{fig:osmdisk10p_inserts}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.23\textwidth}
%         \centering
%         \includegraphics[scale=0.3]{images/disk/osmBP_queries.png}
%         \caption{$OSM-$\bepsilontree{} v/s. \bepsilontree{} Inserts}
%         \label{fig:osmdisk10p_lookups}
%     \end{subfigure}
%     \caption{$OSM-B^+$-tree offers great speedups during inserts but draws an overhead during point lookups 
%     due to the \pinBufName{} }
% \label{fig:osmdisk10p}
% \end{figure}

% \Paragraph{\sysName{}'s query overhead for point queries carries over to disk}
% Point lookups with the same experimental setup as for inserts on disk, carries a similar overhead to the 
% in-memory experiments, as seen in figure ~\ref{fig:osmdisk10p_lookups}. There exists a $1.2\times$ speedup for completely sorted data, primarily due to the faster 
% interpolation search performed in that case as the entire \pinBufName{} contains sorted elements. As we increase the 
% noise in the workload, the performance dips significantly because we spend more time in filtering the appropriate zones 
% and sequentially scanning them. This overhead increases as we move towards more scrambled workloads. 

% \Paragraph{\sysName{}'s performance \TODO{does something} when the buffer size changes}
% Perform experiment when buffer size is decreased. This should technically reduce the speedup in inserts but also 
% decrease the overhead in queries. This will make a case for an adaptive buffer that changes size depending on the 
% read-write workload distribution. 

% \Paragraph{Bloom filter helps reduce the number of query failures}
% \sysName{} employs a Bloom filter (BF) in the \pinBufName{} to reduce unnecessary 
% scans during point lookups for keys that may not exist in the buffer. 
% We utilize a workload of different noise levels with $3\%$ $L$-window that is inserted into 
% an $OSM+$\bplustree{} configuration, and execute $10\%$ random existing queries. 
% Figure ~\ref{fig:bfuse} categorizes the number of queries that would be executed without the BF 
% and also shows the reduction in queries using the BF. Clearly, the BF helps limit the number of unncessary 
% sequential scans in the \pinBufName{} that would otherwise add an additional overhead to the query performance.  

% \begin{figure}[t!]
% 	\centering
%     \includegraphics[width=\columnwidth]{images/BF/bf_use.png}
%     \caption{Number of queries with/without the use of BF in $OSM+$\bplustree{}
%     for a workload with $3\%$ L-window}
% \label{fig:bfuse}
% \end{figure}

==> old-text/motivation.tex <==
It is expected that with increase in sortedness of data, 
the faster the algorithm should sort the data. The most common in-memory sorting algorithms 
like Quicksort have an average runtime of $O(nLogn)$ with the worst case of $O(n^2)$.
However, these algorithms rarely account for nearly sorted data and are not adaptive 
to take advantage of the order present in the data. Ben-Moshe \cite{Ben-Moshe2011} layed out 
an adaptive sorting algorithm that sorts a $(k,l)$-nearly sorted collection in at most two 
sequential passes, and if the algorithm is not $(k,l)$-nearly sorted. It is observed that this 
algorithm performs considerably well over a wide range of \textit{near-sortedness} as discussed 
further in section 6.

$B+$-trees are popular tree based indexes that have been widely studied and adopted. Many attempts
have been made to remodel the $B+$-tree to optimize for different workloads or throughput. One such 
variant is the $B^\epsilon$-tree which was discussed in the previous section. An $\epsilon = 1/2$ 
balances between read and write throughputs in the $B^\epsilon$-tree where the tree is better optimized 
for writes. It is presumed that $B^\epsilon$-tree performs better with inserts due to its buffer, though 
variations in implementation techniques might show otherwise. In such cases, statistics of internal tree 
operations like splits/flushes might better signify performance gains. A bulk-loaded $B+$-tree performs 
the best since data is sorted before performing inserts, thereby 
limiting the I/Os required during build and it is easier to control the fill-factor in the leaf 
pages. A detailed performance analysis of the two different tree indexes is described in section 6 (to be done). 

Studying the architecture of both these tree indexes brings an intuition that the order of data is unaccounted
for while performing inserts in the tree, unless we perform bulk-loading. Not all applications recieve data in 
its entirety before performing inserts. In such cases, it is required to come up with a efficient insert mechanism 
for the popular tree-based indexes. $B^\epsilon$-trees provide a good starting point with the buffer, and our 
proposal looks to exploit the buffer further to capture the near-sorted property in data. 


==> old-text/old-intro.tex <==
\subsection{Problem Statement}
Data can be available in many different forms like streams, collections etc. These data forms also can be quantified by an order that exists during 
retrieval as either completely ordered (ascending/descending), near-sorted or completely scrambled. The first and the last metric have been studied 
extensively, and often serve as best and worst case scenarios for many algorithms, however it is the near-sorted data that needs more attention as 
the world learns more about Big Data. \textit{Pre-Sortedness} is existing order in the data and \textit{Near-sortedness} is when the existing order 
in the data is close to being completely ordered/sorted. In simple terms, the more near-sorted the data is, the closer it is to complete ordering. 
Near-sortedness has been described by many metrics like Inversions, Exchanges, Longest Ascending Subsequence, among others, where all the metrics 
define the data to be close to complete ordering with respect to a certain attribute (discussed in detail under section \ref{sec:presortedness_metrics}). 
Despite the existence of several metrics, there has been very little efforts to nail down on one widely accepted term, thus near-sorted data is often 
quantified and dealt with on a case-by-case basis. 
 
 Popular sorting algorithms like Quicksort, Insertion sort, Bubble sort, as well as popular indexing techniques like the B-trees and $B+$-trees rely on 
 existing ordering in their data, with completely ordered data often being their best cases. There are a few sorting algorithms that are aimed at 
 establishing complete order in nearly-sorted data, but are not popular or do not contain a well described comparisons to existing sorting algorithms. 
 The lack of a well-defined metric has also resulted in indexing techniques to almost ignore the near-sorted cases, with little detail and analysis on 
 their performance against near-sorted data.
 
 \subsection{Motivation}
 Studying the different \textit{near-sortedness} metrics can help in understanding those that capture useful information regarding the distribution of given data. 
 As such, a simple intuition would be that the most beneficial metric would capture maximum information as possible. Nailing down such a metric is crucial in creating 
 a family of differently sorted collections to analyze with sorting algorithms and data structures. 
 
 Analyzing the family of differently sorted collections with various sorting algorithms is key to understanding their performance paradigm with existing algorithms. 
 Few in-memory algorithms exhibit certain traits with specific ordering in the data, and adaptive sorting algorithms are optimized for nearly-sorted data. 
 Studying the behavior of these algorithms with differently sorted data collections would offer deeper insights into the rationale behind performance variations 
 and other characteristcs. 
 
 Existing data structures, mainly indexes like $B+$-trees are popular due to their ability to establish order where the worst-case performance is pretty comparable 
 to the best-case performance. As per textbook implementations, these indexes perform the same irrespective of ordering in data. So, is pre-sortedness/near-sortedness 
 used while inserting elements into the index? Are the computations for near-sorted data and unordered data different? 
 
 Zonemaps are index-like structures where data is located in partitions and reduces the cost for querying. Assuming unique elements, if the data is completely sorted, 
 a point query (existing) will effectively pin-point to a particular partition/zone and perform a search (can do binary since the data within zones is also sorted). 
 Near-sorted data introduces some amount of noise in the collections in the form of misplaced entries, and the effect of this introduced noise on query performance 
 remains to be seen. 

 \subsection{Contributions}
This paper contributes to the above mentioned problem as follows: 
\begin{enumerate}
    \item Identifying information captured by different metrics of pre-sortedness and near-sortedness and decoding the particular metric that would be most useful 
    for quantifying near-sortedness. 
    
    \item Create a family of differently sorted collections using the metric described previously, essentially creating multiple datasets with varying noise levels. 
    
    \item Study performance of sorting algorithms with the multiple collections to analyze their behavior with near-sorted data. 
    
    \item Study the performance of tree based indexes with near-sorted data identifying bottlenecks and trends that account for amortizing the insert costs. 
    
    \item Explore performance of in-memory zonemaps with near-sorted data to understand the effect of partitioning data into zones and study the effect of 
    near-sortedness on zonemap lookups. Additionally, visualize the overlap of minimum and maximum elements in the different zones.  
    
\end{enumerate}


==> old-text/osm-architecture.tex <==
\subsection{$OSM$-$B$-tree}
The $B$-tree approach is based on a vanilla implementation of 
the $B^\epsilon$-tree as shown in Figure \ref{fig:b-epsilon_tree_with_buffer}.
Our idea is to add an additional buffer on top of the $B^\epsilon$-tree
to which elements are first inserted. After reaching a certain threshold
or when the buffer is full, a fraction of elements are then flushed into 
the tree where they are appended at the last level of the $B^\epsilon$-tree. 
We flush the fraction of elements with a certain probability of success that 
they are sorted in-order, with our theory attributed to the data's near-sorted 
property. The key decisions that would be explored are: 
\begin{enumerate}
    \item How much should the buffer be filled before being flushed (threshold)
    \item What fraction of the elements of the buffer should be flushed (a fixed size)
    \item What would be the advantages to this approach as opposed to a bulk loaded $B^epsilon$-tree
\end{enumerate}

\begin{figure}[h!]
    \centering
    \includegraphics[scale=0.50, width=0.5\textwidth]{images/b-epsilon_tree_with_buffer.jpg}
    \Description{$B^\epsilon$-tree with buffered approach}
    \caption{$B^\epsilon$-tree with additional buffer flushed after attaining certain threshold}
    \label{fig:b-epsilon_tree_with_buffer}
\end{figure}

\subsection{$OSM$-$LSM$-tree}
The LSM tree would follow a similar as the $B^\epsilon$-tree as shown in Figure \ref{fig:lsm_tree_with_buffer}. 
We place a buffer (different from $C_0$ level of the LSM-tree), to which elements are 
added as they come in. As and when a certain threshold is reached or the buffer is full, 
the elements will be flushed into the LSM tree and appended at the last level with a 
probabilistic belief that they are sorted in-order. Similar design decisions as the $B$-tree 
also apply to the LSM-tree implementation. In case of an occurence of overlapping value when the 
buffer is full, we present two options that will be explored: 
\begin{enumerate}
    \item Merge with the same file that contains overlapping value.
    \item Create a new file and append to the log.
\end{enumerate}

\begin{figure}[h!]
        \centering
        \includegraphics[scale=0.50, width=0.5\textwidth]{images/lsm_tree_with_buffer.jpg}
        \Description{LSM-tree with buffer}
        \caption{LSM-tree with buffer flushed and appended to the last level}
        \label{fig:lsm_tree_with_buffer}
\end{figure}

==> osm-tree/background.tex <==
\section{Background}
\label{sec:background}

%In this section we define the data sortedness, describe the design of 
%popular 
%indexing data structures and the effect of sortedness on those indexes.

In this section we provide the necessary background for the paper. We first define data sortedness, 
then discuss the sorting algorithms that can exploit sortedness and finally, we introduce the baseline index
data structures that used in our study. Further, we also revisit the concept of \emph{bulk loading}, that acts as 
an ideal baseline to compare our system.  

\Paragraph{Sortedness}
To define sortedness, we refer to the arrival order of the indexed key upon ingestion. 
The arrival order can be \textit{completely-sorted} - where data is arriving completely in-order; 
\textit{near-sorted} - where data is arriving mostly in order albeit with a minor 
fraction of out-of-place elements; or \textit{completely-scrambled} - where data is arriving completely  
out-of-order. 
There is a plethora of proposed metrics to quantify data sortedness \cite{Mannila1985}. 
The most popular metrics include: 
\emph{Inversions}, that tracks the 
number of pairs in incorrect order; \emph{Runs}, that enumerates the number of 
contiguous ordered sub-sequences; \emph{Exchanges}, that calculates the minimum 
number of element exchanges required to bring a list to a sorted 
state~\cite{Mannila1985}. Throughout this paper we use the \emph{(K,L)} 
metric ~\cite{Ben-Moshe2011} that defines near-sorted data in terms of number 
of out-of-place elements and roughness in sorting. In this metric,
$K$ captures the number of unordered elements, and $L$ captures the window 
through which elements may be shuffled within the domain. 

\Paragraph{Sorting Algorithms}
Sorting algorithms can be classified based 
on their \emph{adaptability}, i.e. the algorithm's complexity changes based on pre-sorted input.
The most efficient and widely used sorting algorithm is Quicksort ~\cite{Knuth1998}, 
which is an adaptive sorting algorithm, 
however, it cannot exploit any degree of near-sortedness in the data stream. In fact, if 
the data is entirely sorted, Quicksort can be detrimental if either the first or last element in the 
data stream are chosen as pivots. Recent work on adaptive sorting algorithms have instead,
focused on exploitng any near-sortedness in the data stream to establish order efficiently ~\cite{Ben-Moshe2011}. 
% In this work, we use two different sorting algorithms to order the data:
% an \emph{adaptive sorting algorithm} that takes advantage of near sortedness 
% to reduce sorting cost, and Quicksort when adaptive sorting is not feasible. 

\Paragraph{\emph{$\text{(K,L)}$ Sorting Algorithm}}
The algorithm proposed by Ben-Moshe ~\cite{Ben-Moshe2011} 
sorts a $(K,L)$-near sorted collection in at most two 
sequential passes. The first pass collects the set of misplaced 
entries and the subsequent pass involves placing the misplaced/collected tuples in their correct locations (merge phase). 
As defined above, $K$ is the number of out-of-order entries in the stream, 
while $L$ defines the roughness in sorting. Suppose we have $N$ entries to sort, then
the algorithm takes $O(N \cdot log(K+L))$ computations and uses memory of size $O(K+L)$ to sort the data stream.



%\subsubsection{Inversions (Inv)}
%Manilla \cite{Mannila1985} described inversions as the number of pairs in 
%incorrect order. Assuming ascending order, 
%inversions $Inv(X) = | { (i,j) | 1 \leq i < j \leq n, x_i > x_j } |$. Also, 
%$ 
%0 
%\leq Inv(X) \leq n(n-1)/2 $ for all $X$, 
%with the smallest value fo $Inv(X)$ occuring in case of a completely sorted 
%list and the largest value in case of a list 
%in the opposite order (descending). Though widely studied and used, it has a 
%major drawback that inputs of type 
%$(n+1, n+2, \ldots, 2n, 1, 2, \ldots, n)$ yield a quadratic number of 
%inversions, though they are almost in order and can 
%be sorted easily by dividing the list into two equal halves and merging the 
%first after the second half. 

%\subsubsection{Runs}
%Runs can be simplified as the number of contiguous increasing subsequences 
%of 
%$X$ and \cite{Mannila1985} defines 
%$Runs(X) = | \{ i | 1 \leq i < n $, $a_{i+1} < a_i\}$ $ | + 1$, where 
%$Runs(X) 
%= 1$ or $n$ when the list is already sorted or 
%is in reverse order respectively. This measure also comes with a drawback 
%that 
%local disorder  produces a lot of runs, 
%though the sequence can be easily sorted through bubblesort. 
%
%\subsubsection{Longest Ascending Subsequence (LAS) and Rem}
%The longest ascending subsequence can be visualized as an extension of the 
%previous metric (Runs), signifying the length 
%of the longest run of $X$. \cite{Mannila1985} defines Longest Ascending 
%Subsequence as 
%$Las(X) = max\{ t | \exists i(1), \ldots, i(t), 1 \leq i(1) < \ldots < i(t) 
%\leq n, x_{i(1)} < \ldots < x_{i(t)} \}$ and 
%$Rem(X) = n - Las(X)$ that signifies the number of elements to be removed 
%from 
%X to achieve complete order in the list. 
%$Rem(X) = 0$ or $n-1$ based on whether the list is sorted or in reverse 
%order. 
%
%\subsubsection{Exchanges (Exc)}
%Exchanges are defined by \cite{Mannila1985} as the smallest number of 
%exchanges 
%of arbitrary elements needed to bring $X$
%into ascending order. So, $Exc(X) = 0$ for a completely ordered list and 
%$Exc(X) \leq inv(X)$ for all $X$. The upper bound 
%of exchanges takes into the number of cycles in the permutation ${1, \ldots, 
%n}$ for $X$. Every permutation has at least 
%one cycle so $Exc(X) \leq n - 1$ for all $X$. 
%
%\subsubsection{Enchroaching Lists (EL)}
%Consider an ordered list $l$, with $head(l)$ being the smallest element in 
%$l$ 
%and $tail(l)$ the largest element in $l$. 
%An \textit{encroaching list} set is an ordered set of \textit{ordered lists} 
%$l_1, \ldots l_m$, such that 
%$head(l_i) \leq head(l_{i+1})$ and $tail(l_i) \geq tail(l_{i+1})$ for $1 
%\leq 
%i 
%< m$. The size of this list set $m$ is 
%dependent on the measure of pre-sortedness and thus can be used to quantify 
%the 
%degree of sortedness of data. This size 
%increases with increasing randomness in data \cite{Skiena1988}. 
%
%\subsubsection{(k,l)- nearly sorted}
%Ben-Moshe defined nearly sorted relations with respect to two parameters $k$ 
%and $l$ \cite{Ben-Moshe2011}. The number of 
%unordered elements where captured by $k$ and the window through which 
%elements 
%could be shuffled within the domain was 
%captured by $l$. On a simpler note, $l$ tells us how rough is the sorting or 
%how far elements can be from their actual 
%ordered position, and $k$ tells us how many such elements are out of place.

\Paragraph{\emph{\bplustree{}}}
We focus on on the popular \bplustree{} index data structure that is designed to 
store data in storage. The \bplustree{} keeps part/all of the 
internal nodes using caching in the form of a bufferpool or the file system cache for efficient data access.
We use the \bplustree{} as a "blackbox" for our proposed index design and also compare the performance 
of our design against the textbook \bplustree{}.

% \bplustree{}s are index data structures that store (key,value) pairs. 
A \bplustree{} has one root node, a number of internal nodes and leaf nodes. 
Data pointers are only stored in the leaf nodes, and each 
leaf node is linked to its successor to provide ordered access. The keys of respective 
values stored in the leaf nodes are used as pivot pointers in the internal nodes 
to act as a medium of 
control for querying records or other operations. The
insertion and point-lookup 
cost for the \bplustree{} is $O(log_F (N))$, where $F$ is the fanout 
in the tree and $N$ is the number of leaf pages. 

% \Paragraph{\emph{\bepsilontree{}}}
% $B^\epsilon$-tree is a write-optimized data structure proposed by Brodal 
% and Fagerberg \cite{Brodal2003} as \bplustree{}s with buffers (shown in Figure 
% \ref{fig:b_epsilon_tree}). Every node has 
% a buffer, where inserts are delayed and propagated to lower levels whenever there is an
% overflow. Elements in the buffer of a node are then moved to that of a child node. 
% The buffer improves the I/O bound for inserts 
% without sacrificing query performance. The space allocated for the buffer is controlled
% by a tuning parameter $\epsilon \in [0,1]$. When $\epsilon = 1$, the \bepsilontree{} 
% is simply a \bplustree{}. The 
% insert and read cost are similar to the \bplustree{} but a factor of 
% $\epsilon$. Generally, the insertion cost is $O\left(\frac{log_B (N)}{\epsilon 
% B^{1-\epsilon}}\right)$ and the read cost is $O\left(\frac{log_B (N)}{\epsilon}\right)$, where 
% $B$ is the block size (w.r.t the number of entries stored in a leaf node). 
% If $\epsilon = \frac{1}{2}$, then the cost of 
% insertion becomes $O\left(\frac{log_B (N)}{\sqrt{B}}\right)$ and the read cost becomes 
% $O(2 \cdot log_B (N))$. 

% \begin{figure}[!htb]
% 	\centering
% 	\includegraphics[width=0.9\linewidth]{images/bepsilon_tree.png}
% %	\vspace{-0.25in}
% %	\Description{$B^\epsilon$-tree}
% 	\caption{$B^\epsilon$-tree}
% 	\label{fig:b_epsilon_tree}
% %	\vspace{-0.1in}
% \end{figure} 

% \paragraph{Bloom Filter}
% Bloom Filter (BF) ~\cite{Bloom1970} is a probabilistic, space-efficient data structure used to test  
% the existence of an element in a member set. It carries a possibility of false positive, 
% but guarantees the non-existence of false negatives. The false positive rate increases as elements 
% are added. Theoretically, a BF uses an $m$-bit vector and $k$ independent hash functions to store $n$ 
% elements that can be queried. The expected false positive rate ($f_p$) for 
% optimal number of hash functions ($k_{opt}$) is shown in eq. ~\ref{bloomFalsePositive}:
% \begin{equation}
% 	\label{bloomFalsePositive}
% 	k_{opt} = \ceil{\frac{m}{n}ln2} 
% 	f_p \approx (1 - e^{-\frac{kn}{m}})^k
% \end{equation}

\Paragraph{Bulk Loading}
\label{sec:bulkloading}
When building an index, if we know that the dataset is \emph{completely sorted}, we can bulk load the data into 
the index.\emph{Bulk loading} enables building the tree 
  bottom up using fewer I/Os while operating on sorted data and building the tree nodes in batches. 
 Though this process builds the tree faster than traditional inserts, its drawback is that it requires 
 access to the complete dataset ahead of time. This limits its use 
 for modern applications where newer data needs to be constantly inserted and accessed. 
%\subsubsection{LSM-tree}



==> osm-tree/discussion-learned.tex <==
%\subsection{Learned Indexes}
%\label{subsec:learned}



==> osm-tree/discussion-strings.tex <==
%\subsection{Strings}
%\label{subsec:strings}



==> osm-tree/discussion.tex <==
\section{Discussion}
\label{sec:discussion}

% \mycomment{talk about OSM on other designs -- specifically LSM and Be}

\input{osm-tree/discussion-strings.tex}
\input{osm-tree/discussion-learned.tex}

